Seismic wavefield solutions via physics-guided generative neural operator

Current neural operators often struggle to generalize to complex, out-of-distribution conditions, limiting their ability in seismic wavefield representation. To address this, we propose a generative neural operator (GNO) that leverages generative diffusion models (GDMs) to learn the underlying statistical distribution of scattered wavefields while incorporating a physics-guided sampling process at each inference step. This physics guidance enforces wave equation-based constraints corresponding to specific velocity models, driving the iteratively generated wavefields toward physically consistent solutions. By training the diffusion model on wavefields corresponding to a diverse dataset of velocity models, frequencies, and source positions, our GNO enables to rapidly synthesize high-fidelity wavefields at inference time. Numerical experiments demonstrate that our GNO not only produces accurate wavefields matching numerical reference solutions, but also generalizes effectively to previously unseen velocity models and frequencies.

==> Sections/Acronyms.tex <==
\makeglossaries
\newacronym{gcd}{GCD}{Greatest Common Divisor}
\newacronym{lcm}{LCM}{Least Common Multiple}


==> Sections/Headers.tex <==
% Page headers
\pagestyle{fancy}
\fancyhf{}
\rhead{DW0064  --  09 / 02 / 2025}
% \lhead{\raisebox{-0.5\height}{\includegraphics[height=17mm]{Figures/DigLogo.eps}}}
\lhead{\raisebox{-0.5\height}{\includegraphics[height=17mm]{Figure/DeepWave.png}}}
\rfoot{P\thepage}


% Title
\title{\vspace{5mm}\fontsize{18pt}{20pt}\selectfont\textbf{Physics-guided generative neural operator for seismic wavefield solutions}} 

\author{
\large
\textsc{Shijun Cheng\textsuperscript{1}, Mohammad H. Taufik\textsuperscript{1}, Tariq Alkhalifah\textsuperscript{1}}\\[2mm]
\large \textsuperscript{1}King Abdullah University of Science and Technology, Thuwal, Kingdom of Saudi Arabia
%\vspace{2mm}
}
\date{}



==> Sections/Keywords.tex <==
% Keywords
\keywords{Generative neural operator, Generative diffusion models, Seismic wavefield solutions, Physics guidance}

==> Sections/Symbols.tex <==
\makenomenclature
\nomenclature{\(c\)}{Speed of light in a vacuum}
\nomenclature{\(h\)}{Planck constant}
